Efficient and Robust Long-Form Speech Recognition with Hybrid H3-Conformer

Recently, Conformer has achieved state-of-the-art performance in many speech recognition tasks. However, the Transformer-based models show significant deterioration for long-form speech, such as lectures, because the self-attention mechanism becomes unreliable with the computation of the square order of the input length. To solve the problem, we incorporate a kind of state-space model, Hungry Hungry Hippos (H3), to replace or complement the multi-head self-attention (MHSA). H3 allows for efficient modeling of long-form sequences with a linear-order computation. In experiments using two datasets of CSJ and LibriSpeech, our proposed H3-Conformer model performs efficient and robust recognition of long-form speech. Moreover, we propose a hybrid of H3 and MHSA and show that using H3 in higher layers and MHSA in lower layers provides significant improvement in online recognition. We also investigate a parallel use of H3 and MHSA in all layers, resulting in the best performance.

==> tables/unseen/online_csj_H3_S4.tex <==
\begin{table}[H]
    \centering
    \caption{CER (\%) of offline speech recognition on CSJ}
    \label{table:S4}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccc|ccc}
    \hline
    \multicolumn{2}{c|}{model} & \multicolumn{3}{c|}{short-form} & \multicolumn{3}{c}{long-form}\\
    model & size & eval1 & eval2 & eval3 & eval1 & eval2 & eval3 \\
    \hline
    \hline
    Causal Conformer & 23.7M & \textbf{8.65} & 6.36 & 7.09  & 10.20 & 8.07 & 8.62 \\
    Causal H3-Conformer & 24.0M & 8.87 & \textbf{6.17} & 6.99 & \textbf{9.50} & \textbf{6.74} & \textbf{7.20} \\
    Causal S4-Conformer & 22.5M & 9.02 & 6.50 & \textbf{6.95} & 9.64 & 6.96 & 7.48 \\
    \hline
    \end{tabular}
    }
    

\end{table}


==> tables/unseen/online_csj_chunksize.tex <==
\begin{table}[H]
    \centering
    \caption{Variation of CER (\%) with respect to chunk size}
    \label{table:chunk}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|ccc|ccc}
    \hline
    chunk size & \multicolumn{3}{c|}{Causal Conformer} & \multicolumn{3}{c}{Causal CH4} \\
    & eval1 & eval2 & eval3 & eval1 & eval2 & eval3 \\
    \hline
    \hline
    1 & 8.65 & 6.36 & 7.09 & 8.78 & 6.26 & 6.96 \\
    4 & 8.74 & 6.66 & 7.12 & 8.75 & 6.49 & 6.82 \\
    8 & 8.91 & 6.95 & 7.37 & 8.87 & 6.49 & 6.93 \\
    16 & 9.66 & 7.68 & 8.00 & 8.90 & 6.49 & 6.91 \\
    24 & 10.20 & 8.07 & 8.62 & 9.04 & 6.44 & 6.99 \\
    \hline
    \end{tabular}
    }
\end{table}

==> tables/unseen/online_csj_section.tex <==
\begin{table}[H]
    \centering
    \caption{CER(\%) for each section of recognition results}
    \label{table:MSCER}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|ccc|ccc}
    \hline
    section & \multicolumn{3}{c|}{Causal Conformer[\%]} & \multicolumn{3}{c}{Causal CH4[\%]}\\
    & eval1 & eval2 & eval3 & eval1 & eval2 & eval3 \\
    \hline
    \hline
    1-6 & 7.73 & 6.12 & 6.69 & 7.81 & 5.52 & 6.11 \\
    7-12 & 8.35 & 6.98 & 6.90 & 7.37 & 5.90 & 5.83 \\
    13-18 & 8.89 & 7.89 & 8.59 & 7.93 & 5.89 & 6.32 \\
    19-24 & 10.00 & 7.78 & 8.27 & 7.60 & 5.36 & 5.95 \\
    \hline
    \end{tabular}
    }
\end{table}


==> tables/unseen/online_libri_speed.tex <==
\begin{table}[H]
    \centering
    \caption{Comparison of processing time for long-form speech recognition}
    \label{table:speed}
    \resizebox{\linewidth}{!}{

    \begin{tabular}{r|ccc}
    \hline
    size & \begin{tabular}{c} Causal \\ Conformer \end{tabular} & \begin{tabular}{c} Causal \\ CH4 \end{tabular} & \begin{tabular}{c} Causal \\ H3-Conformer \end{tabular} \\
    & [$\times 10^{-3}$] & [$\times 10^{-3}$] & [$\times 10^{-3}$] \\
    \hline
    \hline
    1 & \textbf{3.220} & 4.457 & 4.689 \\
    4 & 1.467 & \textbf{1.233} & 1.250 \\
    8 & 3.120 & 0.983 & \textbf{0.742} \\
    16 & 6.211 & 1.366 & \textbf{0.618} \\
    24 & 8.914 & 1.938 &  \textbf{0.640} \\
    \hline
    \end{tabular}
    }
    
    
\end{table}

==> texts/acknowledgements.tex <==
I would like to thank my advisor, Professor Tatsuya Kawahara, for his guidance in conducting this research and writing this paper.
I express my deepest gratitude to him. 
I would also like to thank Mr. Shinsuke Sakai and other members of the Speech and Audio Processing Lab for their valuable contributions.


==> texts/related-works/first/SSM-ASR.tex <==
As a previous study applying SSM to ASR tasks, Miyazaki et al. introduced the S4 module into the decoder of the Conformer model\cite{S4-Decoder}.
This approach has been shown to improve the recognition accuracy degradation for long-from ASR in the Conformer.

As a precedent for ASR using both SSM and Self-Attention simultaneously, Saon et al.\cite{DSS-ASR} proposed a model 
in which the depth convolution layer of Conformer is replaced by Diagonal State Spaces (DSS)\cite{DSS}.



==> texts/related-works/first/short-H3.tex <==
H3 is a model proposed by Fu et al.\cite{H3} that uses SSMs for the kernel function of the Linear-Attention model\cite{Linear-Attention}, 
thus enhancing the associative recall capability while reducing computational complexity.

Let the length of the input be L and the query/key/value tokens be $Q_i,K_i,V_i \in \mathbb{R}^{d}(1 \le i \le L)$.
For the similarity function $\mathrm{Sim}: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$, which corresponds to the softmax function in attention, if it can be expressed as $\mathrm{Sim}(q,k)=\phi(q)^T\phi(k)$, the following expression is obtained.
\begin{align}\label{eq:Linear-Attention}
    O_i = \frac{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j){V_j}^T}{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j)}
\end{align}
If $S_i = \sum_{j=1}^{i} \phi(K_j){V_j}^T$, $z_i = \sum_{j=1}^{i} \phi(K_j)$, $O_i$ can be expressed as follows.
\begin{align}\label{eq:Linear-Attention_replace}
    O_i = \frac{\phi(Q_i)^T S_i}{\phi(Q_i)^T z_i}
\end{align}
where $S_i$ and $z_i$ can be computed fast in advance by cumulative summing.
Linear-Attention\cite{Linear-Attention} uses such a method called the inverse kernel trick to calculate attention at high speed.
H3 incorporates SSM into Linear-Attention by replacing $\phi(K_j)$ in the numerator of the expression \ref{eq:Linear-Attention} with $SSM_{shift}$ 
and the sum $S_i$ with $SSM_{diag}$. It can be expressed by the following equation.
\begin{align}
    \bm{Q}\odot\mathrm{SSM_{diag}}(\mathrm{SSM_{shift}(\bm{K})}\odot\bm{V})
\end{align}
where $\odot$ denotes the Adamar product.
The computation of $\mathrm{SSM_{diag}}$ and $\mathrm{SSM_{shift}}$ can be performed with a computational complexity of $O(NL\log L)$, 
and the computational complexity of the entire H3 can be reduced to $O(N^2L+NL\log L)$.
Since the computational complexity of general Self-Attention is $O(NL^2)$, 
it can be said that H3 can suppress the increase in computational complexity for an increase in input length $L$.
Note that $\mathrm{SSM_{diag}}$ is the SSM that restricts the matrix $\bm{A}\in\mathbb{R}^{N \times N}$ to a diagonal matrix 
and $\mathrm{SSM_{shift}}$ is the SSM that restricts the matrix $\bm{A}$ is the SSM restricted to the shift matrix/
$\mathrm{SSM_{shift}}$ can store when a particular event occurred at a past $n$ time by constructing a new internal state based on $\bm{A}\bm{x}_{t-1}$, 
a shift of each component of the internal state at the previous time by one.
Also $\mathrm{SSM_{diag}}$ is the same as S4D by Gu et al.\cite{S4D}. $SSM_{diag}$ can store the state over the entire input series.

H3 has been shown to perform better in natural language processing tasks when hybridized with the attention layer.
Such performance gains from hybridization with the attention layer with a state space model have also been reported for Gated State Spaces (GSS)\cite{GSS} by Mehta et al.

==> texts/related-works/first/short-SSM.tex <==
In the state-space representation, 
the following equation defines the mapping from the input signal series $\bm{U}=(u_1,...,u_L)$ to the output signal series $\bm{Y}=(y_1,...,y_L)$.
\begin{align} \label{eq:SSM_base}
    \begin{split}
        \bm{x}_t = \bm{A}\bm{x}_{t-1} + \bm{B}u_t\\
        y_t = \bm{C}\bm{x}_t + \bm{D}u_t
    \end{split}
\end{align}
where, $\bm{A}\in\mathbb{R}^{m \times m},\bm{B}\in\mathbb{R}^{m \times 1},\bm{C}\in\mathbb{R}^{1 \times m},\bm{D}\in\mathbb{R}^{1 \times 1}$.
Also $\bm{x}_t(0\le t \le L)$ is the internal state vector at each time step.
In the expression \ref{eq:SSM_base}, if $\bm{x}_{-1}=0$, $\bm{x}$ can be eliminated and expressed as follows.
\begin{align}
    \begin{split}
        y_k&=\bm{C}(\bm{A})^k\bm{B}u_0+\cdots+\bm{C}\bm{B}u_k+\bm{D}u_k
    \end{split}
\end{align}
Let $\mathcal{K}_L$ be as follows.
\begin{align} \label{eq:Conv}
    \mathcal{K}_L(\bm{A},\bm{B},\bm{C})=(\bm{C}\bm{B},\bm{C}\bm{A}\bm{B},...,\bm{C}\bm{A}^{L-1}\bm{B})
\end{align}
Then, $\bm{Y}$ can be expressed by convolution.
\begin{align} \label{eq:SSM_y}
    \bm{y}=\mathrm{SSM}(\bm{u})=\mathcal{K}_L(\bm{A},\bm{B},\bm{C})*\bm{u}+\bm{D}\bm{u}
\end{align}
This eliminates the recursive computation and speeds up the process.
In S4, a representative SSM, the class of $\bm{A}$ is restricted to a diagonal matrix plus a low-rank matrix, called a Diagonal Plus Low-Rank (DPLR) representation.
This restriction allows S4 to reduce the computational complexity of the convolution in the expression \ref{eq:Conv} from $O(N^3L)$ to $O(N+L\log L)$.

==> texts/related-works/unseen/H3.tex <==
One advantage of SSM is that, unlike Transformer, 
it is theoretically faster because the computational complexity is roughly linearly proportional to the input length.

However, SSMs have had the problem of slow actual processing speed due to inefficient use of hardware such as GPUs.
In addition, SSMs such as S4D are significantly inferior to Attention in tasks that evaluate the ability to retrieve past tokens, 
such as Induction Head and Associative Recall\cite{AssociativeRecall} using synthetic languages. 
Thus, a difference exists between previous SSMs and Attention in terms of expressive power.

Hungry Hungry Hippos(H3) by Fu et al. was proposed to solve these problems\cite{H3}.
H3 replaces the kernel function of Linear-Attention with SSM.

When the input length is $L$ and there exists query/key/value tokens $Q_i,K_i,V_i \in \mathbb{R}^{d}(1 \le i \le L)$,
Using the similarity function $\mathrm{Sim}: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$, Attention can be expressed as follows.
\begin{align}
    O_i = \frac{\sum_{j=1}^{i} \mathrm{Sim}(Q_i, K_j)V_j}{\sum_{j=1}^{i} \mathrm{Sim}(Q_i, K_j)}
\end{align}
Here, by using a function that can be expressed as $\mathrm{Sim}(q,k)=\phi(q)^T\phi(k)$ instead of the softmax function used in Transformer, 
we obtain the following formula.
\begin{align}\label{eq:Linear-Attention}
    O_i = \frac{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j){V_j}^T}{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j)}
\end{align}
If $S_i = \sum_{j=1}^{i} \phi(K_j){V_j}^T$、$z_i = \sum_{j=1}^{i} \phi(K_j)$, $O_i$ can be expressed as follows.
\begin{align}\label{eq:Linear-Attention_replace}
    O_i = \frac{\phi(Q_i)^T S_i}{\phi(Q_i)^T z_i}
\end{align}
where $S_i$ and $z_i$ can be computed fast in advance by cumulative summing.
Linear-Attention uses such a method called the inverse kernel trick to calculate Attention at high speed.
H3 incorporates SSM into Linear-Attention by replacing $\phi(K_j)$ in the numerator of the expression\ref{eq:Linear-Attention} with $SSM_{shift}$ 
and the sum $S_i$ with $SSM_{diag}$. It can be expressed by the following equation.
\begin{align}
    \bm{Q}\odot\mathrm{SSM_{diag}}(\mathrm{SSM_{shift}(\bm{K})}\odot\bm{V})
\end{align}
where $\odot$ denotes the Adamar product.
The computation of $\mathrm{SSM_{diag}}$ and $\mathrm{SSM_{shift}}$ can be performed with a computational complexity of $O(N+L\log L)$, 
and the computational complexity of the entire H3 can be reduced to $O(N^2L+NL\log L)$.
Since the computational complexity of general Self-Attention is $O(NL^2)$, 
it can be said that H3 can suppress the increase in computational complexity for an increase in input length $L$.
Note that $\mathrm{SSM_{diag}}$ is the SSM that restricts the matrix $\bm{A}\in\mathbb{R}^{N \times N}$ to a diagonal matrix 
and $\mathrm{SSM_{shift}}$ is the SSM that restricts the matrix $\bm{A}$ is the SSM restricted to the shift matrix as follows.
\begin{align}
    \bm{A}_{ij}=
    \begin{cases}
        1 & \text{if } i - 1 = j \\
        0 & \text{if } i - 1 \ne j
    \end{cases}
\end{align}
The $\mathrm{SSM_{shift}}$ can store when a particular event occurred at a past $n$ time by constructing a new internal state based on $\bm{A}\bm{x}_{t-1}$, 
a shift of each component of the internal state at the previous time by one.
Also $\mathrm{SSM_{diag}}$ is the same as S4D by Gu et al.\cite{S4D}.
S4D is a simplification in S4 that restricts the matrix $\bm{A}$ to a diagonal matrix, 
but with appropriate initialization, it is possible to obtain nearly equivalent performance as S4, 
and the same initialization is used in $\mathrm{SSM_{diag}}$.
Since $\bm{A}^n=O$ when $\bm{A}$ is the shift matrix, $SSM_{shift}$ cannot remember inputs older than $n$ times.
On the other hand, this equation does not hold when $\bm{A}$ is a diagonal matrix, so $SSM_{diag}$ can store the state over the entire input series.

H3 has been shown to perform better in benchmarks on natural language processing tasks when used in hybrid form in combination with the Attention layers, 
compared to Transformer alone or H3 alone.
This hybridization of a state space model and Attention layers to improve performance has also been reported in Gated State Spaces (GSS) by Mehta et al.\cite{GSS}.

==> texts/related-works/unseen/SSM.tex <==
In the state-space representation, 
the following equation defines the mapping from the input signal series $\bm{U}=(u_1,...,u_L)$ to the output signal series $\bm{Y}=(y_1,...,y_L)$.
\begin{align} \label{eq:SSM_base}
    \begin{split}
        \bm{x}_t = \bm{A}\bm{x}_{t-1} + \bm{B}u_t\\
        y_t = \bm{C}\bm{x}_t + \bm{D}u_t
    \end{split}
\end{align}
where, $\bm{A}\in\mathbb{R}^{m \times m},\bm{B}\in\mathbb{R}^{m \times 1},\bm{C}\in\mathbb{R}^{1 \times m},\bm{D}\in\mathbb{R}^{1 \times 1}$.
Also $\bm{x}_t(0\le t \le L)$ is the internal state vector at each time step.
Such a model can be expressed as shown in the figure\ref{SSM}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/image_SSM.eps}
    
    \caption{Conceptual diagram of the state-space model}\label{SSM}
\end{figure}


In the High-Order Polynomial Projection Operator (HiPPO) by Gu et al., the pioneer of modern SSM, 
a theoretical formulation of the memory model provides a unified understanding of existing models 
and eliminates implicit dependence on input length and time scale to handle arbitrary length dependencies within the input signal\cite{HiPPO}.

First, when the signal is continuous, by approximating the input signal $f$ with a particular orthogonal polynomial representation, 
such as a Chebyshev polynomial, the past history of the input signal up to time $t$ is represented by a finite set of coefficients $c(t)=(c_0,.... ,c_{N-1})$.
This $c(t)$ can be interpreted as a "memory" at time $t$.
Furthermore, the time expansion of $c(t)$ based on the input at the next time can be expressed as the following ordinary differential equation.
\begin{align} \label{eq:ODE}
    c'(t)=-\frac{1}{t}\widetilde{\bm{A}}(t)c(t)+\frac{1}{t}\widetilde{\bm{B}}(t)f(t)
\end{align}
where, $\widetilde{\bm{A}}(t)\in\mathbb{R}^{N \times N}, \widetilde{\bm{B}}(t)\in\mathbb{R}^{N \times 1}$.

Under certain assumptions, each component of $\widetilde{\bm{A}}$ and $\widetilde{\bm{B}}$ is as follows.
\begin{align}
    \widetilde{A}_{nk} = 
\begin{cases} 
(2n+1)^{\frac{1}{2}}(2k+1)^{\frac{1}{2}} & \text{if } n > k \\
n+1 & \text{if } n = k \\
0 & \text{if } n < k
\end{cases}\\
\widetilde{B}_n = (2n+1)^{\frac{1}{2}}
\end{align}
Integrating both sides of equation\ref{eq:ODE} from $t$ to $t+\Delta t$ yields,
\begin{align}
    c(t+\Delta t)-c(t)=\int_{t}^{t+\Delta t}{ \left \{ -\frac{1}{t}\widetilde{\bm{A}}(t)c(t)+ \frac{1}{t}\widetilde{\bm{B}}(t)f(t) \right \} dt}
\end{align}

Discretizing as $\bm{x}_{k}=c(t+\Delta t),\, \bm{x}_{k-1}=c(t)$, we obtain the following asymptotic formula.
\begin{align}
    \bm{x}_{k}=\bm{A}\bm{x}_{k-1}+\bm{B}u_k
\end{align}
where, $\bm{A}=I-\frac{\widetilde{\bm{A}}}{k},\, \bm{B}=\frac{\widetilde{\bm{B}}}{k}$.

This method is called HiPPO-Legs, and by introducing the HiPPO-Legs discrete-asymptotic formula into RNN, it outperforms existing methods including Transformer.

Linear State-Space Layers (LSSL) by Gu et al.\cite{LSSL} is an extension of HiPPO based on the state-space representation formula\eqref{eq:SSM_base}.
In the expression \eqref{eq:SSM_base}, if $\bm{x}_{-1}=0$, $\bm{x}$ can be eliminated and expressed as follows.
\begin{align}
    \begin{split}
        y_0&=\bm{C}\bm{B}u_0+\bm{D}u_0\\
        y_1&=\bm{C}(\bm{A}\bm{B}u_0+\bm{B}u_1)+\bm{D}u_1\\
        y_2&=\bm{C}(\bm{A}(\bm{A}\bm{B}u_0+\bm{B}u_1)+\bm{B}u_2)+\bm{D}u_2\\
        ...\\
        y_k&=\bm{C}(\bm{A})^k\bm{B}u_0+\bm{C}(\bm{A})^{k-1}\bm{B}u_1+\cdots+\bm{C}\bm{B}u_k+\bm{D}u_k
    \end{split}
\end{align}
Let $\mathcal{K}_L$ be as follows.
\begin{align} \label{eq:Conv}
    \mathcal{K}_L(\bm{A},\bm{B},\bm{C})=(\bm{C}\bm{B},\bm{C}\bm{A}\bm{B},...,\bm{C}\bm{A}^{L-1}\bm{B})
\end{align}
Then, $\bm{Y}$ can be expressed by convolution.
\begin{align} \label{eq:SSM_y}
    \bm{y}=\mathrm{SSM}(\bm{u})=\mathcal{K}_L(\bm{A},\bm{B},\bm{C})*\bm{u}+\bm{D}\bm{u}
\end{align}
This eliminates the recursive computation and speeds up the process.
In addition to make $\bm{A},\bm{B},\bm{C},\bm{D}$ trainable without leaving the HiPPO framework, 
the class of $\bm{A}$ is restricted to a diagonal matrix plus a low-rank matrix, called a Diagonal Plus Low-Rank (DPLR) representation.
This is called S4, which uses the restriction on the class of the matrix $\bm{A}$ 
to reduce the computational complexity of the convolution in the formula\eqref{eq:Conv} from $O(N^3L)$ to $O(N+L\log L)$.

S4 is also known for being the first to solve a task called PATH-X with accuracy superior to random choice in Long-Range Arena \cite{LongRA}, 
a benchmark for uniformly evaluating performance in understanding and processing long-range dependencies.

==> texts/related-works/unseen/short-H3-old.tex <==
H3 is a model proposed by Fu et al.\cite{H3} that uses SSMs for the kernel function of the Linear-Attention model\cite{Linear-Attention}, 
thus enhancing the associative recall capability while reducing computational complexity.

When the input length is $L$ and there exists query/key/value tokens $Q_i,K_i,V_i \in \mathbb{R}^{d}(1 \le i \le L)$,
Using the similarity function $\mathrm{Sim}: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$, Attention can be expressed as follows.
\begin{align}
    O_i = \frac{\sum_{j=1}^{i} \mathrm{Sim}(Q_i, K_j)V_j}{\sum_{j=1}^{i} \mathrm{Sim}(Q_i, K_j)}
\end{align}
Here, by using a function that can be expressed as $\mathrm{Sim}(q,k)=\phi(q)^T\phi(k)$ instead of the softmax function used in Transformer, 
we obtain the following formula.
\begin{align}\label{eq:Linear-Attention}
    O_i = \frac{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j){V_j}^T}{\phi(Q_i)^T \sum_{j=1}^{i} \phi(K_j)}
\end{align}
If $S_i = \sum_{j=1}^{i} \phi(K_j){V_j}^T$, $z_i = \sum_{j=1}^{i} \phi(K_j)$, $O_i$ can be expressed as follows.
\begin{align}\label{eq:Linear-Attention_replace}
    O_i = \frac{\phi(Q_i)^T S_i}{\phi(Q_i)^T z_i}
\end{align}
where $S_i$ and $z_i$ can be computed fast in advance by cumulative summing.
Linear-Attention uses such a method called the inverse kernel trick to calculate Attention at high speed.
H3 incorporates SSM into Linear-Attention by replacing $\phi(K_j)$ in the numerator of the expression \ref{eq:Linear-Attention} with $SSM_{shift}$ 
and the sum $S_i$ with $SSM_{diag}$. It can be expressed by the following equation.
\begin{align}
    \bm{Q}\odot\mathrm{SSM_{diag}}(\mathrm{SSM_{shift}(\bm{K})}\odot\bm{V})
\end{align}
where $\odot$ denotes the Adamar product.
The computation of $\mathrm{SSM_{diag}}$ and $\mathrm{SSM_{shift}}$ can be performed with a computational complexity of $O(N+L\log L)$, 
and the computational complexity of the entire H3 can be reduced to $O(N^2L+NL\log L)$.
Since the computational complexity of general Self-Attention is $O(NL^2)$, 
it can be said that H3 can suppress the increase in computational complexity for an increase in input length $L$.
Note that $\mathrm{SSM_{diag}}$ is the SSM that restricts the matrix $\bm{A}\in\mathbb{R}^{N \times N}$ to a diagonal matrix 
and $\mathrm{SSM_{shift}}$ is the SSM that restricts the matrix $\bm{A}$ is the SSM restricted to the shift matrix/
$\mathrm{SSM_{shift}}$ can store when a particular event occurred at a past $n$ time by constructing a new internal state based on $\bm{A}\bm{x}_{t-1}$, 
a shift of each component of the internal state at the previous time by one.
Also $\mathrm{SSM_{diag}}$ is the same as S4D by Gu et al.\cite{S4D}. $SSM_{diag}$ can store the state over the entire input series.

H3 has been shown to perform better in natural language processing tasks when hybridized with the Attention layer.
Such performance gains from hybridization with the Attention layer with a state space model have also been reported for Gated State Spaces (GSS)\cite{GSS} by Mehta et al.
